Streaming, Memory Limited Matrix Completion with Noise

In this paper, we consider the streaming memory-limited matrix completion problem when the observed entries are noisy versions of a small random fraction of the original entries. We are interested in scenarios where the matrix size is very large so the matrix is very hard to store and manipulate. Here, columns of the observed matrix are presented sequentially and the goal is to complete the missing entries after one pass on the data with limited memory space and limited computational complexity. We propose a streaming algorithm which produces an estimate of the original matrix with a vanishing mean square error, uses memory space scaling linearly with the ambient dimension of the matrix, i.e. the memory required to store the output alone, and spends computations as much as the number of non-zero entries of the input matrix.

==> intro.tex <==
\section{Introduction}

Reconstructing a structured (e.g. low rank) matrix from noisy observations of a subset of its entries constitutes a fundamental problem in collaborative filtering \cite{rennie2005}, and has recently attracted much interest, see e.g. \cite{candes2009exact}, \cite{candes2010power}, \cite{keshavan2010matrix}, \cite{recht2011simpler}. The recent development of matrix completion algorithms has been largely motivated by the design of efficient recommendation systems. These systems (amazon, netflix, google) aim at proposing items or products from large catalogues to targeted users based on the ratings provided by users of a small subset of items. This goal naturally translates to a matrix completion problem where the rows (resp. the columns) of the matrix correspond to items (resp. to users). And often, the (item, user) rating matrix is believed to exhibit a low rank structure due to the inherent similarities among users and among items. 

In this paper, we address the problem of matrix completion in scenarios where the matrix can be extremely large, so that (i) it might become difficult to manipulate or even store, and (ii) the complexity of the proposed algorithms should not rapidly increase with the matrix dimensions. In other words, we aim at designing matrix completion algorithms under memory and computational constraints. Memory-limited algorithms are particularly relevant in the streaming data model, where observations (e.g. ratings in recommendation systems) are collected sequentially. We assume here that the columns of the matrix are revealed one by one to the algorithm. More specifically, a subset of noisy entries of an arriving column is observed, and may be stored, but the algorithm cannot request these entries later if they were not stored. The streaming model seems particularly appropriate to model recommendation systems, where users actually seek for recommendations sequentially. Recently, motivated by the need to understanding high-dimensional data, several machine learning techniques, such as PCA \cite{mitliagkas2013} or low-rank matrix approximation \cite{clarkson2009numerical}, have been revisited considering memory and computational constraints. To our knowledge, this paper provides the first analysis of the matrix completion problem under these constraints (refer to the related work section for a detailed description of the connection of our problem to existing work).

%Imagine that there are $m$ movies and $n$ users and each user rates a
%small part of movies what she or he has watched through a service
%provider such as Netflix. Of course, the service provider will want to
%build a movie recommandation system using the rating data, which is
%often called {\em collaborative filtering}. The {\em collaborative
 % filtering} is equivalent to the {\em matrix completion}
%problem. Movie-User ratings generate a $m\times n$ matrix where rows
%and columns correspond to users and movies and only a small
%fraction of entries has the rating information. Finding the hidden values
%of the rating matrix, we can make a nice recommandation
%system. While there are many different matrices having different
%values for the missing entries, the matrix is commonly believed
%low-rank (It is widely believed that only a few factors decide the
%rating scores), and from the low-rank property, we might find the ground
%truth matrix which has the exact users' rating scores for all movies.

%Here, we consider scenarios where the data size can be extremely large
%so that the rating matrix between users and movies could be extremely
%difficult to manipulate and store. Recently, we have already entered
%the ``big data'' era and the growing speed of the data size is much
%faster than the improvement speeds of memory space and computing
%power. Therefore, we study matrix completion problems with limited
%memory space and computational complexity. Memory limited algorithms
%are relevant in the streaming data model, where observations are
%collected sequentially. We assume here that at each time a user
%arrives to the memory limited system and gives ratings of some movies,
%which is equivalent to the case that the columns of the rating matrix
%are revealed one by one to the algorithm.

Throughput the paper, we use the following notations. For any $m\times n$ matrix $A$, we denote by $A^\dagger$ its transpose. We also denote by $s_1(A)\geq \dots \geq  s_{n\wedge m}(A)\geq 0$, the singular values of $A$. The SVD of matrix $A$ is $A=U\Sigma V^{\dagger}$ where $U,V$ are unitary matrices and $\Sigma = \mbox{diag}(s_1(A),\dots s_{n\wedge m}(A))$. $A^{-1}$ denotes the Pseudo-inverse matrix of $A$, i.e. $ A^{-1} = V \Sigma^{-1}U^\dagger$. Finally, for any vector $v$, $\| v\|$ denotes its Euclidean norm, whereas for any matrix $A$, $\|A
  \|_F$ denotes its Frobenius norm, $\|A\|_2$ its operator norm, and $\|A\|_\infty$ its $\ell_\infty$-norm, i.e., $\|A\|_\infty=\max_{i,j}|A_{ij}|$.

\medskip
\noindent
{\bf Contributions.} Let $M\in [0,1]^{m\times n}$ denote the $m\times n$ ground-truth matrix we wish to recover from noisy observations of some of its entries. $M$ is assumed to exhibit a {\it sparse structure} (refer to Assumption 1 (i) for a formal definition). $m$ and $n$ are typically very large, and can be thought as tending to $\infty$. The SVD of $M$ is $M=U \Lambda V^{\dagger} $. We assume that each entry of $M$ is observed (but corrupted by noise) with probability $\delta$ (independently over entries). The random set of observed entries is denoted by $\Omega$, and we introduce the following operator from $\mathbb{R}^{m\times n}$ to itself: for all $Y\in\mathbb{R}^{m\times n}$,  
$$
[\mathcal{P}_{\Omega}(Y)]_{ij} = \begin{cases} Y_{ij}, \quad & \mbox{if}\quad
  (i,j)\in \Omega \cr 0,& \mbox{otherwise} .\end{cases} 
  $$
Then, we wish to reconstruct $M$ from the observed matrix $A = \mathcal{P}_{\Omega}(M+X)$, where $X$ is a noise matrix with independent and zero-mean entries, and such that $M_{ij}+X_{ij} \in [0,1]$. Note that $\delta$ typically depends of $n$ and $m$, and tends to zero as $n$ and $m$ tend to infinity. Finally, we analyze the matrix completion problem under the {streaming model:} we assume that in each round, a column of $A$ is observed. This column is uniformly distributed among the set of columns that have not been observed so far. 

We present SMC (Streaming Matrix Completion), a memory-limited and low-complexity algorithm which, based on the observed matrix $A$, constructs an estimator $\hat{M}$ of $M$. We prove, under mild assumptions on $M$ and the proportion $\delta$ of observed entries, that $\hat{M}$ is {\it asymptotically accurate}, in the sense that its average mean-square error converges to 0 as both $n$ and $m$ grows large, i.e., $\frac{\|\hat{M}-M \|_F^2}{mn} = o(1)$. More precisely, we make the following assumption. 

\medskip
\noindent
{\it Assumption 1.} (i) (Structural sparsity of $M$) There exists $k\leq \min(n,m)$ such that $\frac{s_k(M)}{s_{k+1}(M)}=\omega(1)$ and $\sum_{i=k+1}^{K}s_{i}^2(M) = o(mn)$.  (ii) $\delta = \omega (k \max({1\over n},\frac{\log^2 m}{ m}))$, and  $\delta = o(\frac{1}{k \log^2 m})$.

\medskip
\noindent
The main result of this paper is a direct consequence of Theorems~\ref{thm:stmcomp}, \ref{thm:memory}, and \ref{thm:complex}. It states that under {Assumption 1}, with high probability, the SMC algorithm provides an asymptotically accurate estimate $\hat{M}$ of $M$ using one pass on the observed matrix $A$, and requires $O(km+kn)$ memory space and $O(\delta mn k)$ operations.

Note that Assumption 1 (i) is satisfied as soon as $M$ has low rank. More precisely, when rank$(M)=K$, then (i) is satisfied when $k=K$. In such a case, there is a non-empty set of sampling rates $\delta$ for which SMC yields an asymptotically accurate estimate of $M$ as soon as $K=o({\sqrt{m}\over \log(m)^2})$ (if for example $m$ and $n$ grows at the same pace to infinity). 

%The objective of this work is to find a memory efficient and low
%complexity algorithm which reconstructs $M$ {\em asymptotically
 % accurately}. More precisely, we propose an algorithm which finds
%a $m\times K$ matrix $\hat{U}$ and a $n\times K$ matrix $\hat{V}$ such that
%$\frac{\|\hat{U}\hat{V}^\dagger -M \|_F^2}{mn} = o(1)$ with
%$O(Km+ Kn)$ memory space, $O(\delta m n K)$ computations and 1-pass
%streaming input.


%\subsection{Our results}
%Many papers dealing with matrix completion consider memory usage or
%computational complexity. The related works in the previous part
%introduce many beautiful theories to reduce memory space or
%computational complexity under some performance constraints. Although the
%algorithms work very well with any input matrix, there are still a
%huge room to improve when the input streaming matrix is sparse.

The SMC algorithm consists in three main steps. In the first step, 

\noindent{\bf \em Algorithm overview:} We fully exploit the sparsity of
the input matrix.
\begin{itemize}
\item At first, we store $\ell$ arriving columns into the
memory space. Because of the sparsity, when $\ell = O(\delta
(m+n)/\log m)$, the required memory space to store $\ell$ columns is
$O(m+n)$. While such $\ell$ is not enough to find principle column
vectors, we can reconstruct $K$ principle row vectors for the $m\times
\ell$ submatrix of $M$ corresponding to the arriving columns
(Theorem~\ref{pro:pca}). 
\item Let $A^{(B)}$ denote the first $\ell$ arriving vectors and
  $Q^\dagger$ be the $K$ principle row vectors reconstructed from
  $A^{(B)}$. Using $Q$ and $A^{(B)}$, we generate $K$ reference column
  vectors $W = A^{(B)} \cdot Q$. Although the columns of $W$ are not
  the principle column vectors of $M$, they are very useful. Indeed,
  $A$ has $K$ strong singular values which are much larger than others
  and stem from $M$. Therefore, $\hat{V} = A^\dagger \cdot W$ amplifies
  the part of $W$ sharing the same column space with $M$ a lot more
  than the remaining part. In the sequel, the rows of
  $\hat{V}^\dagger$ become very close to the principle row vectors of
  $M$ (Theorem~\ref{thm:streamingV}).
\item Once we know $\hat{V}^\dagger$ of which rows are very close to the principle row
  vectors of $M$, it is very easy to find
  column vectors $\hat{U}$ such that
  $\frac{\|\hat{U}\hat{V}-M\|_F^2}{mn}=o(1)$. Using the Gram-Schmidt
  process, we can easily find $\hat{R}$ such that $\hat{V}\hat{R}$ is an orthonormal
  matrix and $\hat{U} = \frac{1}{\delta}A \hat{V} \hat{R} \hat{R}^\dagger$ is the
  solution since $\hat{U}\hat{V}^\dagger = \frac{1}{\delta} A \hat{V}
  \hat{R} (\hat{V} \hat{R})^\dagger$ where $\hat{V}
  \hat{R} (\hat{V} \hat{R})^\dagger$ is the projection matrix onto the
  linear span of the rows of $M$.
\end{itemize}
For this algorithm, 1-pass streaming input is enough. For the
streaming input, we can sequentially compute $\hat{V}^j = A_j^\dagger
W$ and update $\hat{U} =
(\sum_{i=1}^{n} A_i \hat{V}^i )\cdot \hat{R} \hat{R}^\dagger$ where $\hat{R}
\hat{R}^\dagger$ can be computed after we get $\hat{V}$. Therefore, we do
not need to store columns to find $\hat{V}$ and $\hat{U}$ for the
1-pass streaming input except the first $\ell$ arriving columns.

\iffalse
\section{Related Work}

This section surveys existing work on the design of matrix completion algorithms. We also provide a description of recent work on rank-$k$ approximation and PCA algorithms, as these algorithms could be seen as building blocks of matrix completion methods. The section is organised as follows. We first review algorithms for matrix completion. We then focus on streaming algorithms for rank-$k$ approximation, and PCA. Finally we discuss algorithms designed to be computationally efficient. 

\medskip
\noindent
{\bf Matrix completion algorithms.} \cite{candes2009exact} first showed that in absence of noise
(i.e., $X=0$), the matrix $M$, with low rank $k$, can be recovered exactly using convex relaxation under some conditions on the sampling rate $\delta$ and the singular vectors. These conditions were improved in\cite{candes2010power} and \cite{recht2011simpler}. The proposed algorithms involves solving a convex program, which can be computationally expensive. If the rank $k$ of the matrix is known, $M$ can be recovered using simpler spectral methods. For example, in \cite{keshavan2010matrix}, the authors show that $M$ can be reconstructed asymptotically accurately 



 showed that
finding the $K$ largest singular values and corresponding singular
vectors is enough to reconstruct $M$. With $O(\delta K mn \log n )$
operations, the spectral method finds $\hat{M}$ such that
$\frac{\|M-\hat{M}\|_F^2}{mn} = o(1)$ when $\delta m = \omega(1)$ and
$\delta n = \omega(1)$. Such $\hat{M}$ can be found with noisy
observations as well. \cite{candes2010matrix} and
\cite{keshavan2009matrix} showed that both the nuclear norm minimization
and the spectral method are asymptotically accurate algorithms, respectively. 


\subsubsection*{Streaming algorithms}

\cite{clarkson2009numerical} proposed a rank $K$ approximation
algorithm with 1-pass streaming input, where they exploited a subspace
embedding technique with the Rademacher matrix in order to save memory
space. They showed that the algorithm uses
$O(K\varepsilon^{-1}(m+n) \log (mn))$ memory space and the output
$\hat{A}^{(K)}$ satisfies
\begin{equation} 
\|A- \hat{A}^{(K)} \|_F \le (1+\varepsilon)\|A- \bar{A}^{(K)} \|_F,\label{eq:con1}\end{equation}
where $\bar{A}^{(K)}$ is the optimal rank $K$ approximation. However,
the memory space is superlinear to $m+n$ and the Frobenius norm bound
does not guarantee the asymptotically accurate reconstruction. For the
matrix completion problem, the condition \eqref{eq:con1} can guarantee
at most
$\|\hat{M}-M\|_F^2 = O( \frac{\varepsilon^2}{\delta}mn)$ and thus we
need $\varepsilon = \omega(\sqrt{1/\delta})$ for asymptotically
accurate reconstruction.

We can also use streaming PCA algorithms to reconstruct $M$, although
they cannot finish the matrix completion with 1-pass streaming. Using
the streaming PCA algorithms, we could generate matrix completion
algorithms as follows: first find principle column vectors with 1-pass
or multiple passes streaming input and then find row vectors
corresponding to the principle column vectors with another 1-pass
streaming input. Therefore, we need at least 2-pass streaming input to
finish the matrix completion with the PCA algorithms. The matrix
sketching algorithms are the streaming PCA methods with 1-pass
input. The matrix sketching is first proposed by
\cite{liberty2013simple} and finds the principle column vectors very well
when the input matrix is not sparse. For the sparse input matrices
like the matrix completion problem, the algorithm by
\cite{ghashami2014relative} is a good solution where they first find
$\ell=o(1/\delta)$ columns using the matrix sketching then pick $K$
principle columns from the $\ell$ columns. Thus, the required memory
space is $O(\frac{m}{\delta}+Kn)$.  The streaming PCA by
\cite{mitliagkas2013} is not a matrix sketching algorithm. Instead,
they proposed a block stochastic power method. Although they need
$O(\log m)$-pass streaming input, the required memory space is only
$O(Km+Kn)$.
 
% When arrival pattern is streaming and memory space is limited,
% \begin{itemize}
% \item \cite{balzano2010online}: Every time, they update the principle
%   $K$ column vector to the gradient of the nuclear norm minimization
%   problem 
% \item \cite{liberty2013simple}: Matrix sketching (Frequency direction)
%   algorithm is proposed
% \item \cite{ghashami2014relative}: First, using Frequency direction
%   they get $\ell >> K$ columns and then do rank $K$ approximation.
% \item \cite{mitliagkas2013}: Block stochastic power method is proposed
% \end{itemize} 

\subsubsection*{Low complexity algorithms}
When it comes to computational complexity, many studies have tried to
reduce the matrix dimensions (i.e. $m$ and $n$) since the complexity
scales with the matrix dimensions in general. The randomized numerical
linear algebra is very useful to reduce the matrix demensions. There
is a nice survey paper by \cite{halko2011finding} on the
low complexity low-rank matrix approximation algorithms using the
randomized numerical linear algebra. When the input matrix is not sparse, the Subsampled Randomized
Hadamard Transform (SRHT) is a very popular randomized linear algebra
to reduce the matrix dimension. For instance, \cite{woolfe2008fast},
\cite{boutsidis2013improved}, and \cite{tropp2011improved} use the
SRHT to solve the low rank approximation. When the input matrix is sparse, \cite{clarkson2013low} reduces computational complexity
using a sparse embedding space where the proposed algorithm finds a
rank $K$ approximation $\hat{A}^{(K)}$ satisfying the condition \eqref{eq:con1} with
$O(\delta mn) + O((nK^2\varepsilon^{-4}+K^3\varepsilon^{-5})\cdot
\mbox{polylog}(m+n))$ operations. Since the asymptotically accurate
reconstruction can be achieved with the condition \eqref{eq:con1} and
$\varepsilon^2 = \omega(1/\delta)$, the complexity to say the
asymptotically accurate reconstruction
becomes $\omega(\delta mn K)$ when $m = O(\frac{K}{\delta^3})$.


% \begin{itemize}
% \item \cite{mackey2011distributed}:To reduce computational complexity,
%   they consider divide and conquer algorithms.
% \end{itemize}


% There are other algorithms.
% \begin{itemize}
% \item \cite{mazumder2010spectral}: Reducing computational complexity
%   sum of sparse matrix and low rank matrix. (Soft-impute)
% \item \cite{Dhanjal2014online}: On-line matrix completion based on Soft-impute algorithm
% \end{itemize}


\noindent{\bf More Notations:}
When $A$ and $B$ are matrices having the same number of rows, we simply use
$[A, B]$ to denote the matrix of which columns come from columns of $A$
and $B$ sequentially.
We denote by $A_{\bot}$  an orthonormal basis of the perpendicular space to
  the linear span of the columns of $A$.
We use $A_i$, $A^j$, and $[A]_{ij}$ to denote the $i$-th column of $A$, the
$j$-th row of $A$, and the element of $A$ in
  the $i$-th row and the $j$-th column, respectively. $A^{a:b}$ and
  $A_{a:b}$ indicate submatrices of $A$ from the $a$-th row to the
  $b$-th row and from the $a$-th column to the $b$-th column,
  respectively. 
%We denote by $\lambda_k(A)$ the $k$-th largest singular value of $A$. 
We
  defind a bounding operator for matrices as follows: for all $i$ and $j$
$$[|A|^a_b]_{ij} = \begin{cases} a \quad & \mbox{if}\quad
  [A]_{ij} \ge a ,\cr [A]_{ij}\quad & \mbox{if}\quad a>[A]_{ij}>b,\cr
b \quad & \mbox{if}\quad [A]_{ij}\le b .\end{cases} $$
\fi
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> intro2.tex <==
\section{Introduction}

Reconstructing a structured (e.g. low rank) matrix from noisy observations of a subset of its entries constitutes a fundamental problem in collaborative filtering \cite{rennie2005}, and has recently attracted much interest, see e.g. \cite{candes2009exact}, \cite{candes2010power}, \cite{keshavan2010matrix}, \cite{recht2011simpler}. The recent development of matrix completion algorithms has been largely motivated by the design of efficient recommendation systems. These systems (amazon, netflix, google) aim at proposing items or products from large catalogues to targeted users based on the ratings provided by users of a small subset of items. This goal naturally translates to a matrix completion problem where the rows (resp. the columns) of the matrix correspond to items (resp. to users). And often, the (item, user) rating matrix is believed to exhibit a low rank structure due to the inherent similarities among users and among items. 

In this paper, we address the problem of matrix completion in scenarios where the matrix can be extremely large, so that (i) it might become difficult to manipulate or even store, and (ii) the complexity of the proposed algorithms should not rapidly increase with the matrix dimensions. In other words, we aim at designing matrix completion algorithms under memory and computational constraints. Memory-limited algorithms are particularly relevant in the streaming data model, where observations (e.g. ratings in recommendation systems) are collected sequentially. We assume here that the columns of the matrix are revealed one by one to the algorithm. More specifically, a subset of noisy entries of an arriving column is observed, and may be stored, but the algorithm cannot request these entries later if they were not stored. The streaming model seems particularly appropriate to model recommendation systems, where users actually seek for recommendations sequentially. Recently, motivated by the need to understand high-dimensional data, several machine learning techniques, such as PCA \cite{mitliagkas2013} or low-rank matrix approximation \cite{clarkson2009numerical}, have been revisited considering memory and computational constraints. To our knowledge, this paper provides the first analysis of the matrix completion problem under these constraints (refer to the related work section for a detailed description of the connection of our problem to existing work).

%Imagine that there are $m$ movies and $n$ users and each user rates a
%small part of movies what she or he has watched through a service
%provider such as Netflix. Of course, the service provider will want to
%build a movie recommandation system using the rating data, which is
%often called {\em collaborative filtering}. The {\em collaborative
 % filtering} is equivalent to the {\em matrix completion}
%problem. Movie-User ratings generate a $m\times n$ matrix where rows
%and columns correspond to users and movies and only a small
%fraction of entries has the rating information. Finding the hidden values
%of the rating matrix, we can make a nice recommandation
%system. While there are many different matrices having different
%values for the missing entries, the matrix is commonly believed
%low-rank (It is widely believed that only a few factors decide the
%rating scores), and from the low-rank property, we might find the ground
%truth matrix which has the exact users' rating scores for all movies.

%Here, we consider scenarios where the data size can be extremely large
%so that the rating matrix between users and movies could be extremely
%difficult to manipulate and store. Recently, we have already entered
%the ``big data'' era and the growing speed of the data size is much
%faster than the improvement speeds of memory space and computing
%power. Therefore, we study matrix completion problems with limited
%memory space and computational complexity. Memory limited algorithms
%are relevant in the streaming data model, where observations are
%collected sequentially. We assume here that at each time a user
%arrives to the memory limited system and gives ratings of some movies,
%which is equivalent to the case that the columns of the rating matrix
%are revealed one by one to the algorithm.

Throughout the paper, we use the following notations. For any $m\times n$ matrix $A$, we denote by $A^\dagger$ its transpose. We also denote by $s_1(A)\geq \dots \geq  s_{n\wedge m}(A)\geq 0$, the singular values of $A$. The SVD of matrix $A$ is $A=U\Sigma V^{\dagger}$ where $U$ and $V$ are unitary matrices and $\Sigma = \mbox{diag}(s_1(A),\dots s_{n\wedge m}(A))$. $A^{-1}$ denotes the Pseudo-inverse matrix of $A$, i.e. $ A^{-1} = V \Sigma^{-1}U^\dagger$. Finally, for any vector $v$, $\| v\|$ denotes its Euclidean norm, whereas for any matrix $A$, $\|A
  \|_F$ denotes its Frobenius norm, $\|A\|_2$ its operator norm, and $\|A\|_\infty$ its $\ell_\infty$-norm, i.e., $\|A\|_\infty=\max_{i,j}|A_{ij}|$.

\medskip
\noindent
{\bf Contributions.} Let $M\in [0,1]^{m\times n}$ denote the $m\times
n$ ground-truth matrix we wish to recover from noisy observations of
some of its entries. $M$ is assumed to exhibit a {\it sparse
  structure} (refer to Assumption 1 (ii) for a formal definition). $m$
and $n$ are typically very large, and can be thought as tending to
$\infty$. %The SVD of $M$ is $M=U \Lambda V^{\dagger} $. 
We assume that each entry of $M$ is observed (but corrupted by noise) with probability $\delta$ (independently over entries). The random set of observed entries is denoted by $\Omega$, and we introduce the following operator from $\mathbb{R}^{m\times n}$ to itself: for all $Y\in\mathbb{R}^{m\times n}$,  
$$
[\mathcal{P}_{\Omega}(Y)]_{ij} = \begin{cases} Y_{ij}, \quad & \mbox{if}\quad
  (i,j)\in \Omega \cr 0,& \mbox{otherwise} .\end{cases} 
  $$
Then, we wish to reconstruct $M$ from the observed matrix $A = \mathcal{P}_{\Omega}(M+X)$, where $X$ is a noise matrix with independent and zero-mean entries, and such that $M_{ij}+X_{ij} \in [0,1]$. Note that $\delta$ typically depends of $n$ and $m$, and tends to zero as $n$ and $m$ tend to infinity. Finally, we analyze the matrix completion problem under the {streaming model:} we assume that in each round, a column of $A$ is observed. This column is uniformly distributed among the set of columns that have not been observed so far. 

We present SMC (Streaming Matrix Completion), a memory-limited and low-complexity algorithm which, based on the observed matrix $A$, constructs an estimator $\hat{M}$ of $M$. We prove, under mild assumptions on $M$ and the proportion $\delta$ of observed entries, that $\hat{M}$ is {\it asymptotically accurate}, in the sense that its average mean-square error converges to 0 as both $n$ and $m$ grows large, i.e., $\frac{\|\hat{M}-M \|_F^2}{mn} = o(1)$. More precisely, we make the following assumption. 

\medskip
\noindent
{\it Assumption 1.} (i) $\|M\|^2_F = \Theta(mn)$.\\ (ii) (Structural
sparsity of $M$) there exists $i\leq \min(n,m)$ such that
$\frac{s_i(M)}{s_{i+1}(M)}=\omega(1)$ and $\sum_{j=i+1}^{m\wedge n}s_{j}^2(M) = o(mn)$. We denote by $k$ the smallest $i$ satisfying this condition.\\ (iii) $\delta = \omega (k \max({k\over n},\frac{\log^2 m}{ m},\frac{k\log m}{ m}))$, and  $\delta = o(\frac{1}{\log^2 m})$. 

\medskip
\noindent
The main result of this paper is a direct consequence of Theorems~\ref{thm:stmcomp}, \ref{thm:memory}, and \ref{thm:complex}. It states that under {Assumption 1}, with high probability, the SMC algorithm provides an asymptotically accurate estimate $\hat{M}$ of $M$ using one pass on the observed matrix $A$, and requires $O(km+kn)$ memory space and $O(\delta mn k)$ operations.

Note that Assumption 1 (ii) is satisfied as soon as $M$ has low rank. More precisely, when rank$(M)=K$, then (ii) is satisfied when $k=K$. In such a case, there is a non-empty set of sampling rates $\delta$ for which SMC yields an asymptotically accurate estimate of $M$ as soon as $K=o({\sqrt{m}\over \log(m)^2})$ (if for example $m$ and $n$ grows at the same pace to infinity). 

Note also that $O(km+kn)$ is the dimension of the ambient space for $M$, i.e. $M$ can be well-approximated by a rank$(k)$ matrix and hence $(km+kn)$ is the minimum memory size required to output a good estimate of $M$. Our algorithm SMC is optimal in the sense that it only requires the amount of memory required to store the output.

%The objective of this work is to find a memory efficient and low
%complexity algorithm which reconstructs $M$ {\em asymptotically
 % accurately}. More precisely, we propose an algorithm which finds
%a $m\times K$ matrix $\hat{U}$ and a $n\times K$ matrix $\hat{V}$ such that
%$\frac{\|\hat{U}\hat{V}^\dagger -M \|_F^2}{mn} = o(1)$ with
%$O(Km+ Kn)$ memory space, $O(\delta m n K)$ computations and 1-pass
%streaming input.


%\subsection{Our results}
%Many papers dealing with matrix completion consider memory usage or
%computational complexity. The related works in the previous part
%introduce many beautiful theories to reduce memory space or
%computational complexity under some performance constraints. Although the
%algorithms work very well with any input matrix, there are still a
%huge room to improve when the input streaming matrix is sparse.
\medskip
The SMC algorithm consists in three main steps. 
\begin{itemize}
\item Step 1. We first treat the $\ell = \frac{1}{\delta \log m}$ first arriving columns. These columns do not contain enough information to learn the right singular vectors of $M$ since there are many rows with no observed entries. Instead, we can extract the top $k$ right singular vectors for the submatrix of $M$ corresponding to the $\ell$ arriving columns. Let $A^{(B)}$ be the $\ell$ arriving columns and $Q$ be the top $k$ right singular vectors extracted from the $A^{(B)}$. After finding $Q$, we compute and keep $W=A^{(B)}Q$ for the next step. $W$ will be used to recover the top $k$ right singular vectors of $M$. 

\item Step 2. We extract the top $k$ right singular vectors of $M$ using $W$. We show that the linear span of the columns of $\hat{V} = A^\dagger \cdot W$ is similar to the linear span of the top $k$ right singular vectors of $M$ (Theorem~\ref{thm:streamingV}).  Although $W$ is noisy, the matrix product amplifies the linear span of the top $k$ right singular vectors of $M$.

\item Step 3. Once we know $\hat{V}^\dagger$, it is easy to find column vectors $\hat{U}$ such that
  $\frac{\|\hat{U}\hat{V}-M\|_F^2}{mn}=o(1)$. First, using the Gram-Schmidt
  process, we find $\hat{R}$ such that $\hat{V}\hat{R}$ is an orthonormal
  matrix and compute $\hat{U} = \frac{1}{\delta}A \hat{V} \hat{R} \hat{R}^\dagger$.
  Then, $\hat{U}\hat{V}^\dagger = \frac{1}{\delta} A \hat{V}
  \hat{R} (\hat{V} \hat{R})^\dagger$ where $\hat{V}
  \hat{R} (\hat{V} \hat{R})^\dagger$ is the projection matrix onto the
  linear span of the top $k$ right singular vectors of $M$. Therefore, $\hat{U}\hat{V}^\dagger$ becomes very close to the best rank $k$ approximation.
\end{itemize}

We show that these three steps can be realized in a memory-efficient manner, and using low complexity algorithms.
%For the
%streaming input, we can sequentially compute $\hat{V}^j = A_j^\dagger
%W$ and update $\hat{U} =
%(\sum_{i=1}^{n} A_i \hat{V}^i )\cdot \hat{R} \hat{R}^\dagger$. We do
%not need to store columns to find $\hat{V}$ and $\hat{U}$ for the
%1-pass streaming input except the first $\ell$ arriving columns.

\medskip
\noindent{\bf Additional Notations.} When matrices $A$ and $B$ have
the same number of rows, $[A, B]$ to denote the matrix whose first
columns are those of $A$ followed by those of $B$. For any matrix $A$,
$A_{\bot}$ denotes an orthonormal basis of the subspace perpendicular
to the linear span of the columns of $A$. $A_i$, $A^j$, and $A_{ij}$
denote the $i$-th column of $A$, the $j$-th row of $A$, and the
$(i,j)$ entry of $A$, respectively. For $b\ge a$, $A^{a:b}$ and
$A_{a:b}$ are submatrices of $A$ respectively defined as
$A^{a:b}=(A^j)_{j=a,\ldots,b}$ and
$A_{a:b}=(A_i)_{i=a,\ldots,b}$. Also, we will abbreviate
$A_{1:k}^{1:k}$ to $A_{[k]}$.
Finally, we define the following thresholding operator for matrices. The operator is defined by two real positive numbers $a$ and $b$, with $b\ge a$, and if applied to $A$, it returns the matrix $|A|_a^b$ such that 
$$[|A|^b_a]_{ij} = \begin{cases} b \quad & \mbox{if}\quad
  A_{ij} \ge b ,\cr A_{ij}\quad & \mbox{if}\quad a<A_{ij}<b,\cr
a \quad & \mbox{if}\quad A_{ij}\le a.\end{cases} $$



\section{Related Work}

This section surveys existing work on the design of matrix completion algorithms. We also provide a description of recent work on rank-$k$ approximation and PCA algorithms, as these algorithms could be seen as building blocks of matrix completion methods. The section is organised as follows. We first review algorithms for matrix completion. We then focus on streaming algorithms for rank-$k$ approximation, and PCA. Finally we discuss algorithms designed to be computationally efficient. 

\medskip
\noindent
{\bf Matrix completion algorithms.} \cite{candes2009exact} first showed that in absence of noise
(i.e., $X=0$), the matrix $M$, with low rank $k$, can be recovered exactly using convex relaxation under some conditions on the sampling rate $\delta$ and the singular vectors. These conditions were improved in \cite{candes2010power} and \cite{recht2011simpler}, and the approach was also extended to the case of noisy observed entries \cite{candes2010matrix}. The proposed algorithms involves solving a convex program, which can be computationally expensive. If the rank $k$ of the matrix is known, $M$ can be recovered using simpler spectral methods. For example, in \cite{keshavan2010matrix}, the authors show that in absence of noise, $M$ can be reconstructed asymptotically accurately using $O(\delta k mn \log n )$ operations under the conditions that the rank $k$ does not depend on $n $ and $m$, $\delta m = \omega(1)$ and $\delta n = \omega(1)$. Again these results can be adapted to the presence of noise \cite{keshavan2009matrix}. In this paper, we improve the spectral method used in \cite{keshavan2010matrix} and \cite{keshavan2009matrix}, so that it becomes memory-efficient, and so that it has performance guarantees even if the rank $k$ of $M$ scales with $m$ and $n$.

\medskip
\noindent
{\bf Streaming algorithms.} \cite{clarkson2009numerical} proposes an algorithm to provide a rank-$k$ approximation of a fully observed matrix $A$, using 1-pass on the columns of $A$. The algorithm uses a random $m\times \ell$ Rademacher matrix $S$, with an appropriate choice of $\ell$, and outputs a rank-$k$ matrix $\hat{A}^{(k)}$ constructed from $A^\dagger S$ and $AA^\dagger S$. When setting $\ell = O(k\varepsilon^{-1}\log(1/\eta))$ which requires $O(k\varepsilon^{-1}(m+n)\log(1/\eta))$ memory space, it is shown that with probability at least $1-\eta$,
\begin{equation} 
\|A- \hat{A}^{(k)} \|_F \le (1+\varepsilon)\|A- \bar{A}^{(k)} \|_F,\label{eq:con1}
\end{equation}
where $\bar{A}^{(k)}$ is the optimal rank-$k$ approximation of $A$. We could think of applying this algorithm to our problem. If the observed matrix $A$ is $A={\cal P}_{\Omega}(M+X)$, it would make sense to estimate $M$ by $\frac{1}{\delta}\hat{A}^{(k)}$ where $\hat{A}^{(k)}$ is the output of the algorithm in \cite{clarkson2009numerical} applied to $A$. Indeed, it is easy to check that $\|M-\frac{1}{\delta}\bar{A}^{(k)} \|_F^2 = o(mn)$ (i.e., the optimal rank-$k$ approximation of ${1\over \delta}A$ estimates $M$ asymptotically accurately). However, in general, $\frac{1}{\delta}\hat{A}^{(k)}$ is not asymptotically accurate:
\begin{eqnarray*}
\frac{\|M -\frac{1}{\delta}\hat{A}^{(k)} \|_F^2}{mn} &\ge& \frac{(\|A-
  \hat{A}^{(k)} \|_F - \|A- \bar{A}^{(k)}\|_F-\|\bar{A}^{(k)}- \delta
  M \|_F)^2}{\delta^2 mn}\cr
&= &\frac{(\varepsilon \|A- \bar{A}^{(k)}\|_F-\|\bar{A}^{(k)}- \delta
  M \|_F)^2}{\delta^2 mn}.
\end{eqnarray*}
Now, one can also easily check that $\|A- \bar{A}^{(k)} \|_F = \Theta (\sqrt{\delta mn})$ and $\|\delta M-\bar{A}^{(k)} \|_F = o(\delta \sqrt{mn})$, so that if we choose $\epsilon=\sqrt{\delta}$, we get $\frac{\|M -\frac{1}{\delta}\hat{A}^{(k)} \|_F^2}{mn}=\Omega(1)$. As a consequence, using the algorithm in \cite{clarkson2009numerical}, we cannot reconstruct $M$ asymptotically accurately using $O(k\sqrt{1/\delta}(m+n)\log(1/\eta))$ memory space. Recall that our algorithm reconstructs $M$ accurately with $O(k(m+n))$ memory space.  

We could also think of using sketching and streaming PCA algorithms to reconstruct $M$. When the columns arrive sequentially, these algorithms identify the left singular vectors in 1-pass on the matrix. We would then need a second pass on the data to estimate the right singular vectors, and complete the matrix. For example, \cite{liberty2013simple} proposes a sketching algorithm that updates the $\ell$ most frequent directions when a new column of $A$ is (fully) observed. This algorithm outputs a sketch $\hat{A}$ of $A$ and has the following performance guarantee: $\|A A^\dagger - \hat{A}\hat{A}^{\dagger} \|_2 \le \frac{2\|A\|_F^2}{\ell}$. It also uses $O(m\ell)$ memory space. Again if we apply the algorithm to our matrix completion problem, i.e., to the observed matrix $A={\cal P}_{\Omega}(M+X)$, where $M$ is of rank $k$, then $\|A \|_F^2 = \Theta(\delta m n)$ and $\sigma_k (AA^\dagger ) =\Theta( \delta^2 \sigma_k^2 (M)) = \Theta
(\frac{\delta^2 mn}{k})$. Hence to efficiently extract the top $k$ left singular vectors, we would need that $\frac{2\|A \|_F^2}{\ell} = o(\sigma_k (AA^\dagger ))$, which implies $\ell = \omega(k/\delta)$. Therefore, the required memory space would be $O(\frac{km}{\delta} + kn)$. Our algorithm is more efficient, and uses only 1-pass on the matrix. Note that the streaming PCA algorithm proposed in \cite{mitliagkas2013} does not apply to our problem (in \cite{mitliagkas2013}, the authors consider the spiked covariance model where a column is randomly generated in an i.i.d. every time).


% the algorithm by
% \cite{ghashami2014relative} is a good solution where they first find
% $\ell=o(1/\delta)$ columns using the matrix sketching then pick $K$
% principle columns from the $\ell$ columns. Thus, the required memory
 
% When arrival pattern is streaming and memory space is limited,
% \begin{itemize}
% \item \cite{balzano2010online}: Every time, they update the principle
%   $K$ column vector to the gradient of the nuclear norm minimization
%   problem 
% \item \cite{liberty2013simple}: Matrix sketching (Frequency direction)
%   algorithm is proposed
% \item \cite{ghashami2014relative}: First, using Frequency direction
%   they get $\ell >> K$ columns and then do rank $K$ approximation.
% \item \cite{mitliagkas2013}: Block stochastic power method is proposed
% \end{itemize} 
\medskip
\noindent
{\bf Low complexity algorithms.} There have been recently an intense research effort to propose low-complexity algorithms for various linear algebra problems. Randomization has appeared as an efficient way to reduce the complexity of algorithms, see \cite{halko2011finding} for a survey. For example, \cite{sarlos2006improved} and \cite{clarkson2009numerical} devise algorithms for rank-$k$ approximation with guarantees (\ref{eq:con1}) and that use $O(\delta mn (k/\varepsilon + k \log k) + n\mbox{poly}(k/\varepsilon))$ operations. When the input matrix is sparse, \cite{clarkson2013low} leverages sparse embedding techniques, and reduces the required complexity to $O(\delta mn) + O((nk^2\varepsilon^{-4}+k^3\varepsilon^{-5})\cdot\mbox{polylog}(m+n))$ operations. But once again, as explained above, these results do not apply to our framework ((\ref{eq:con1}) is not enough to guarantee an asymptotically accurate matrix completion).


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> model.tex <==
\section{Model}

\subsection{Notations} 
For the sake of notational simplicity, we use $A^{-1}$
for any size of matrix $A$ to denote the reverse matrix of $A$ or the
Pseudo-inverse matrix~\footnote{$ V
  \Sigma^{-1} U^\dagger$ is the pseudoinverse of $A$ when
  the singular value decomposition of $A$ is $U\Sigma V^{\dagger}$} and
$X^\dagger$ to denote the transpose
  matrix of $X$. When
$A$ and $B$ are matrices having the same number of rows, we simply use
$[A, B]$ to denote the matrix of which columns come from columns of $A$
and $B$ sequentially.
We denote by $A_{\bot}$  an orthonormal basis of the perpendicular space to
  the linear span of the columns of $A$.
We use $A_i$, $A^j$, and $[A]_{ij}$ to denote the $i$-th column of $A$, the
$j$-th row of $A$, and the element of $A$ in
  the $i$-th row and the $j$-th column, respectively. $\lambda_k(A)$
  denotes the $k$-th largest singular value of $A$. For a vector
  $v$, $\| v\|$ denotes its Euclidean norm. For a matrix $A$, $\|A
  \|_F$ is its Frobenius norm and $\|A\|_2$ is its operator norm. We
  defind a bounding operator for matrices as follows: for all $i$ and $j$
$$[|A|^a_b]_{ij} = \begin{cases} a \quad & \mbox{if}\quad
  [A]_{ij} \ge a ,\cr [A]_{ij}\quad & \mbox{if}\quad a>[A]_{ij}>b,\cr
b \quad & \mbox{if}\quad [A]_{ij}\le b .\end{cases} $$

In this work, $\hat{X}$ implies an output matrix
from a random input and $\bar{X}$ implies an expected matrix when the
input is the mean of the random input.  

% \subsection{Community detection with general frame work}
% Consider the Netflix model. Users make ratings for some movies. We can consider a
% community model as follows:
% \begin{itemize}
% \item There are $K$ classes of users
% \item Each user has $L$ dimensional vector and each element has a
%   value in $[0,1]$ (ratings for $L$ movies with continuous value)
% \item $a_u \in [0,1]^{L}$ : the $L$ dimensional vector of user $u$ 
% \item $\mathbb{E}[(a_u)^T a_v] = r_{k(u)k(v)}$ where $k(u)$ and $k(v)$
%   denote the classes of $u$ and $v$, respectively. Thus, there are $K$
%   communities and according to the communities users' vectors are
%   correlated.
% \item $R = (r_{ij})_{1\le i,j \le K}$
% \item $\lambda_k (R)$ : the $k$-th largest singular value of $R$. In
%   this paper $\lambda_{k}(\cdot)$ denotes the $k$-th largest singular
%   value and $\lambda_{\max}(\cdot) = \lambda_{1}(\cdot)$.
% \end{itemize}



% \begin{theorem}
% When $f(n) = \omega(\log n)$,
% $$\|V_{\bot}^{T} \hat{V} \| = O(\frac{f(n)}{\delta \sqrt{mn}}) \quad\mbox{with
%   probability}\quad 1-\exp(-f(n)) .$$
% \end{theorem}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> sec2.tex <==

\section{Related Work}

\subsection{Matrix completion algorithms}
\cite{candes2009exact} showed that when there is no noise
(i.e., $X=0$) $M$ can be recovered exactly. They make a convex
optimization problem and proved that the solution is the same with $M$
under some conditions on $\delta$ and singular vectors. \cite{candes2010power}
and \cite{recht2011simpler} find more tight conditions where
 when $\delta m = \Omega (k\cdot \mbox{polylog}(n))$ and the singular
 vectors are well spread out,
$M$ is the solution of   
\begin{eqnarray}
\min_{\hat{M}} ~~~~& & \|\hat{M} \|_* \cr
\mbox{subject to}& &{P}_{\Omega}(\hat{M}) = A, \label{eq:nm}
\end{eqnarray}
where $\|\hat{M} \|_*$ indicates the nuclear norm of $\hat{M}$.

Although \eqref{eq:nm} is a convex problem, the computational
complexity is still high. When knowing the rank of $M$, we can simply
use spectral methods. \cite{keshavan2010matrix} showed that
finding the $k$ largest singular values of $A$ and corresponding singular
vectors is enough to reconstruct $M$ asymptotically accurately. With $O(\delta k mn \log n )$
operations, the spectral method finds $\hat{M}$ such that
$\frac{\|M-\hat{M}\|_F^2}{mn} = o(1)$ when $k$ is a constant,
$\frac{m}{n}$ is bounded away from 0 and $\infty$, and
$\delta m = \omega(1)$. Such $\hat{M}$ can be found with noisy
observations as well. \cite{candes2010matrix} and
\cite{keshavan2009matrix} showed that both the nuclear norm minimization
and the spectral method are asymptotically accurate algorithms, respectively. 


\subsection{Streaming algorithms}

\cite{clarkson2009numerical} proposed a rank $k$ approximation
algorithm with 1-pass streaming input. Under the algorithm, they
randomly generate a $m\times \ell$ Rademacher matrix $S$, compute
$A^\dagger S$ and $A A^\dagger S$, and reconstruct a rank $k$
approximation $\hat{A}^{(k)}$ from $A^\dagger S$ and $A A^\dagger
S$.
Thus, the algorithm has to memorize the $n \times \ell$ matrix
$A^\dagger S$ and the $m\times \ell$ matrix $A A^\dagger S$. They
showed that the algorithm can reconstruct $\hat{A}^{(k)}$ with
$\ell = O(k\varepsilon^{-1}\log(1/\eta))$ (or with
$O(k\varepsilon^{-1}(m+n)\log(1/\eta))$ memory space) which satisfies
with probability at least $1-\eta$
\begin{equation} 
\|A- \hat{A}^{(k)} \|_F \le (1+\varepsilon)\|A- \bar{A}^{(k)} \|_F,\label{eq:con1}\end{equation}
where $\bar{A}^{(K)}$ is the optimal rank $K$ approximation. However, the condition \eqref{eq:con1} does not imply the asymptotically accurate
reconstruction. For instance, consider that $\varepsilon = \sqrt{\delta}$,
$\|A- \hat{A}^{(k)} \|_F = (1+\varepsilon)\|A- \bar{A}^{(k)} \|_F$,
and the optimal rank $k$ approximation is asymptotically accurate
(i.e., $\|M-\frac{1}{\delta}\bar{A}^{(k)} \|_F^2 = o(mn) $).
Since 
$\|A- \bar{A}^{(k)} \|_F = \Theta (\sqrt{\delta mn})$ under the matrix
completion model and $\|\delta M-\bar{A}^{(k)} \|_F = o(\delta \sqrt{mn}) $, 
from the triangular inequality, 
\begin{eqnarray*}
\frac{\|M -\frac{1}{\delta}\hat{A}^{(k)} \|_F^2}{mn} &\ge& \frac{(\|A-
  \hat{A}^{(k)} \|_F - \|A- \bar{A}^{(k)}\|_F-\|\bar{A}^{(k)}- \delta
  M \|_F)^2}{\delta^2 mn}\cr
&= &\frac{(\varepsilon \|A- \bar{A}^{(k)}\|_F-\|\bar{A}^{(k)}- \delta
  M \|_F)^2}{\delta^2 mn}= \Omega(1),
\end{eqnarray*}
which means that the rank $k$ approximation is not
accurate. Therefore, $O(k\sqrt{1/\delta}(m+n)\log(1/\eta))$ memory
space does not guarantee the asymptotically accurate reconstruction.

We can also use matrix sketching or streaming PCA algorithms to
reconstruct $M$. The algorithms find left singular vectors (principle
column vectors) througout the column-wise streaming input. Using the
algorithms, we could generate a matrix completion algorithm as
follows: first find principle column vectors with 1-pass or multiple
passes streaming input and then find row vectors corresponding to the
principle column vectors with another 1-pass streaming
input. Therefore, we need at least 2-pass streaming input to finish
the matrix completion with the PCA
algorithms. \cite{liberty2013simple} proposed a matrix sketching
algorithm which updates $\ell$ frequent-directions for the 1-pass
streaming input. Under the matrix sketching algorith, the required
memory space is $O(m\ell)$ and the output $\hat{A}$ satisfies that
$\|A A^\dagger - \hat{A}\hat{A}^{\dagger} \|_2 \le \frac{2\|A
  \|_F^2}{\ell}$.
For the matrix completion problem, $\|A \|_F^2 = \Theta(\delta m n)$
and
$\sigma_k (AA^\dagger ) =\Theta( \delta^2 \sigma_k^2 (M)) = \Theta
(\frac{\delta^2 mn}{k})$.
Therefore, $\frac{2\|A \|_F^2}{\ell} = o(\sigma_k (AA^\dagger ))$ if
and only if $\ell = \omega(k/\delta)$, which means that we have to
keep $\omega(1/\delta)$ directions to find the top $k$ left singular
vectors accurately. Therefore, the required memory space is
$O(\frac{km}{\delta} + kn)$.  The streaming PCA by \cite{mitliagkas2013}
is not for the matrix streaming input, but for the spiked covariance
model where a column is generated randomly at every time. The
streaming PCA algorithm uses a block stochastic power method and find
principle column vectors with $O(km+kn)$ space for the spiked covariance
model.


% the algorithm by
% \cite{ghashami2014relative} is a good solution where they first find
% $\ell=o(1/\delta)$ columns using the matrix sketching then pick $K$
% principle columns from the $\ell$ columns. Thus, the required memory
 
% When arrival pattern is streaming and memory space is limited,
% \begin{itemize}
% \item \cite{balzano2010online}: Every time, they update the principle
%   $K$ column vector to the gradient of the nuclear norm minimization
%   problem 
% \item \cite{liberty2013simple}: Matrix sketching (Frequency direction)
%   algorithm is proposed
% \item \cite{ghashami2014relative}: First, using Frequency direction
%   they get $\ell >> K$ columns and then do rank $K$ approximation.
% \item \cite{mitliagkas2013}: Block stochastic power method is proposed
% \end{itemize} 

\subsection{Low complexity algorithms}
When it comes to computational complexity, many studies have tried to
reduce the matrix dimensions (i.e. $m$ and $n$) since the complexity
scales with the matrix dimensions. The randomized numerical linear
algebra is very useful to reduce the matrix demensions, which is well
surveyed in \cite{halko2011finding}. The randomized and approximation
approach can solve the rank $k$ approximation satisfying the condition
\eqref{eq:con1} in
$O(\delta mn (k/\varepsilon + k \log k) + n
\mbox{poly}(k/\varepsilon))$ computations 
\cite{sarlos2006improved} and \cite{clarkson2009numerical}.
% When the input matrix is not sparse, the Subsampled Randomized
% Hadamard Transform (SRHT) is a very popular randomized linear algebra
% to reduce the matrix dimension. For instance, \cite{woolfe2008fast},
% \cite{boutsidis2013improved}, and \cite{tropp2011improved} use the
% SRHT to solve the low rank approximation. 
When the input matrix is sparse, \cite{clarkson2013low} reduces
computational complexity more
using a sparse embedding space where the proposed algorithm finds a
rank $k$ approximation satisfying the condition \eqref{eq:con1} with
$O(\delta mn) + O((nK^2\varepsilon^{-4}+K^3\varepsilon^{-5})\cdot
\mbox{polylog}(m+n))$ operations. Since the asymptotically accurate
reconstruction is not guaranteed by the condition \eqref{eq:con1} and
$\|A- \hat{A}^{(k)} \|_F = (1+\varepsilon)\|A- \bar{A}^{(k)} \|_F$
implies non-accurate reconstruction when  
$\varepsilon \ge \sqrt{\delta}$, the sparse embedding algorithm does
not guarantee the asymptotically accurate reconstruction with
$O(\delta m n k)$ especially when $m = O(\frac{K}{\delta^3})$.


% \begin{itemize}
% \item \cite{mackey2011distributed}:To reduce computational complexity,
%   they consider divide and conquer algorithms.
% \end{itemize}


% There are other algorithms.
% \begin{itemize}
% \item \cite{mazumder2010spectral}: Reducing computational complexity
%   sum of sparse matrix and low rank matrix. (Soft-impute)
% \item \cite{Dhanjal2014online}: On-line matrix completion based on Soft-impute algorithm
% \end{itemize}


\noindent{\bf More Notations:}
When $A$ and $B$ are matrices having the same number of rows, we simply use
$[A, B]$ to denote the matrix of which columns come from columns of $A$
and $B$ sequentially.
We denote by $A_{\bot}$  an orthonormal basis of the perpendicular space to
  the linear span of the columns of $A$.
We use $A_i$, $A^j$, and $[A]_{ij}$ to denote the $i$-th column of $A$, the
$j$-th row of $A$, and the element of $A$ in
  the $i$-th row and the $j$-th column, respectively. $A^{a:b}$ and
  $A_{a:b}$ indicate submatrices of $A$ from the $a$-th row to the
  $b$-th row and from the $a$-th column to the $b$-th column,
  respectively. 
%We denote by $\lambda_k(A)$ the $k$-th largest singular value of $A$. 
We
  defind a bounding operator for matrices as follows: for all $i$ and $j$
$$[|A|^a_b]_{ij} = \begin{cases} a \quad & \mbox{if}\quad
  [A]_{ij} \ge a ,\cr [A]_{ij}\quad & \mbox{if}\quad a>[A]_{ij}>b,\cr
b \quad & \mbox{if}\quad [A]_{ij}\le b .\end{cases} $$

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 

